Autocorrelations and Thermal Fragility of Anyonic Loops in Topologically Quantum Ordered Systems

Are systems that display Topological Quantum Order (TQO), and have a gap to excitations, hardware fault-tolerant at finite temperatures? We show that in surface code models that display low d-dimensional Gauge-Like Symmetries, such as Kitaev's and its generalizations, the expectation value of topological symmetry operators vanishes at any non-zero temperature, a phenomenon that we coined thermal fragility. The autocorrelation time for the non-local topological quantities in these systems may remain finite even in the thermodynamic limit. We provide explicit expressions for the autocorrelation functions in Kitaev's model. If temperatures far below the gap may be achieved then these autocorrelation times, albeit finite, can be made large. The physical engine behind the loss of correlations at large spatial and/or temporal distance is the proliferation of topological defects at any finite temperature as a result of a dimensional reduction. This raises an important question: How may we best quantify the degree of protection of quantum information in a topologically ordered system at finite temperature?

==> ekqc_a.tex <==
\usepackage{calc,ifthen}

\unitlength 1in
\newcommand{\nputbox}[3]{\put(#1){\makebox(0,0)[#2]{#3}}}
\newcommand{\nputgr}[4]{\put(#1){\makebox(0,0)[#2]{\includegraphics[#3]{#4}}}}

\newlength{\elimdepthdim}
\newlength{\elimheightdim}
\newlength{\elimwidthdim}
\newcommand{\elimdepth}[1]{
\setlength{\elimdepthdim}{\depthof{#1}}
\setlength{\elimheightdim}{\heightof{#1}}
\setlength{\elimwidthdim}{\widthof{#1}}
\raisebox{0in}[\elimheightdim][0in]{#1}
}

\newlength{\strutdepthdim}
\newlength{\strutheightdim}
\newlength{\strutwidthdim}
\newcommand{\strutlike}[1]{
\setlength{\strutdepthdim}{\depthof{#1}}
\setlength{\strutheightdim}{\heightof{#1}}
\rule[-\strutdepthdim]{0in}{\strutheightdim+\strutdepthdim}
}
\newcommand{\iboxlike}[1]{%
\setlength{\strutdepthdim}{\depthof{#1}}%
\setlength{\strutheightdim}{\heightof{#1}}%
\setlength{\strutwidthdim}{\widthof{#1}}%
\rule[-\strutdepthdim]{0in}{\strutheightdim+\strutdepthdim}%
\rule{\strutwidthdim}{0in}%
}

\newcommand{\vrulelike}[2]{
\setlength{\strutdepthdim}{\depthof{#1}}
\setlength{\strutheightdim}{\heightof{#1}}
\rule[-\strutdepthdim]{#2}{\strutheightdim+\strutdepthdim}
}

\newcommand{\rrght}{\raggedright}
\newcommand{\fhf}{\hspace*{\fill}}


\def\one{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l} {\rm
1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}

\newcommand{\qvbar}{\mbox{$|\hspace*{-3pt}|\hspace*{-3pt}|$}}
%\hspace*{1pt}\strutlike{\big\{}\vrulelike{\{}{1.1pt}\hspace*{1pt}
\newcommand{\qrangle}{\mbox{$\rangle\hspace*{-4.3pt}\rangle\hspace*{-4.3pt}\rangle$}}
\newcommand{\qlangle}{\mbox{$\langle\hspace*{-4.3pt}\langle\hspace*{-4.3pt}\langle$}}

\newcommand{\sysfnt}{\mathsf}
\newcommand{\qsys}[1]{{\sysfnt #1}}
\newcommand{\ket}[1]{\qvbar{#1}\qrangle}
\newcommand{\bra}[1]{\qlangle{#1}\qvbar}
\newcommand{\braket}[2]{\qlangle{#1}\qvbar{#2}\qrangle}
\newcommand{\ketbra}[2]{\ket{#1}\bra{#2}}
\newcommand{\kets}[2]{\qvbar{#1}\qrangle_{{}_{\!\!\scriptstyle{\sysfnt{#2}}}}}
\newcommand{\bras}[2]{{}^{\scriptstyle\sysfnt{ #2}}\!\qlangle{#1}\qvbar}
\newcommand{\brakets}[3]{{}^{\scriptstyle\sysfnt{ #3}}\!\qlangle{#1}\qvbar{#2}\qrangle_{{}_{\!\!\scriptstyle{\sysfnt{#3}}}}}
\newcommand{\ketbras}[3]{\kets{#1}{#3}\!\!\bras{#2}{#3}}
\newcommand{\slb}[2]{{#1}^{({\sysfnt{#2}})}}


\newcommand{\qavec}[2]{\left(\!\begin{array}{c}#1\\ #2\end{array}\!\right)}
\newcommand{\qaop}[4]{\left(\begin{array}{cc}#1&#2\\ #3&#4\end{array}\right)}

\newcommand{\qbvec}[4]{\left(\!\begin{array}{c}#1\\ #2\\ #3\\ #4\end{array}\!\right)}


\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cZ}{{\cal Z}}
\renewcommand{\tensor}{\otimes}
\newcommand{\trace}{\mbox{tr}}
\newcommand{\vspan}{\mbox{span}}

\def\id{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l} {\rm
1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\newcommand{\suchthat}{{\;\vrulelike{\{}{1.1pt}\;}}

\newcommand{\mbz}{\mathbf{0}}
\newcommand{\mbo}{\mathbf{1}}
\newcommand{\mb}[1]{\mathbf{#1}}

%\newcommand{\uts}[1]{{#1}}
\def\uts#1{{\mathchoice{\mbox{#1}}{\mbox{#1}}{\mbox{\small #1}}{\mbox{\tiny #1}}}\,}

\newcommand{\bitzero}{\mathfrak{0}}
\newcommand{\bitone}{\mathfrak{1}}
\newcommand{\biz}{\bitzero}
\newcommand{\bio}{\bitone}
\newcommand{\bittwo}{\mathfrak{2}}
\newcommand{\bitthree}{\mathfrak{3}}
\newcommand{\bitfour}{\mathfrak{4}}
\newcommand{\bitfive}{\mathfrak{5}}
\newcommand{\bitsix}{\mathfrak{6}}
\newcommand{\bitseven}{\mathfrak{7}}
\newcommand{\stfnt}{\mathfrak}
\newcommand{\idop}{\id}

\newcommand{\zop}{\mathbb{O}}
\newcommand{\rls}{\mathbb{R}}
\newcommand{\cmplx}{\mathbb{C}}
\newcommand{\cmplxp}{\mathbb{CP}}
\newcommand{\matalg}[1]{\mathrm{Mat}_{#1}(\cmplx)}
\newcommand{\real}{\mathrm{Re}}
\newcommand{\imag}{\mathrm{Im}}
\newcommand{\vdim}{\textrm{dim}}

\newcommand{\lie}[1]{\mathfrak{#1}}
\newcommand{\glc}[1]{\mathfrak{gl}_{#1}\cmplx}
\newcommand{\slc}[1]{\mathfrak{sl}_{#1}\cmplx}
\newcommand{\soc}[1]{\mathfrak{so}_{#1}\cmplx}
\newcommand{\spc}[1]{\mathfrak{sp}_{#1}\cmplx}
\newcommand{\glr}[1]{\mathfrak{gl}_{#1}\rls}
\newcommand{\slr}[1]{\mathfrak{sl}_{#1}\rls}
\newcommand{\sor}[1]{\mathfrak{so}_{#1}\rls}
\newcommand{\spr}[1]{\mathfrak{sp}_{#1}\rls}
\newcommand{\cstar}{\dagger}
\newcommand{\scstar}[1]{{#1}^{\!\cstar}}
\newcommand{\trless}[1]{{#1}_{\!\circ}}

\newcommand{\restrict}{{\upharpoonright}}

\newtheorem{Theorem}{Theorem}
\newtheorem{Conjecture}[Theorem]{Conjecture}
\newtheorem{Problem}[Theorem]{Problem}
\newtheorem{Claim}[Theorem]{Claim}
\newtheorem{Lemma}[Theorem]{Lemma}
\newtheorem{Corollary}[Theorem]{Corollary}
\newcommand{\proof}{\paragraph*{Proof.}}
\newcommand{\proofof}[1]{\paragraph*{Proof of Theorem~#1.}}
\newcommand{\qed}{\hspace*{\fill}\rule{2.5mm}{2.5mm}%
\vspace*{8pt}\par}

\newcounter{herefignum}
\newenvironment{herefig}{\begin{center}\refstepcounter{herefignum}}{\end{center}}
\newcommand{\herefigcap}[1]{\\\begin{minipage}{\textwidth}{FIG.~\theherefignum: #1}\end{minipage}}

\newcommand{\itb}{{$\bullet$}}
\newcommand{\itd}{{\raisebox{4pt}{\rule{4pt}{1.5pt}}}}

\newenvironment{titems}{\begin{itemize}%
\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}\setlength{\parskip}{0pt}}{%
\end{itemize}}%

